The Hawkes Edge Partition Model for Continuous-time Event-based Temporal Networks

We propose a novel probabilistic framework to model continuous-time interaction events data. Our goal is to infer the \emph{implicit} community structure underlying the temporal interactions among entities, and also to exploit how the community structure influences the interaction dynamics among these nodes. To this end, we model the reciprocating interactions between individuals using mutually-exciting Hawkes processes. The base rate of the Hawkes process for each pair of individuals is built upon the latent representations inferred using the hierarchical gamma process edge partition model (HGaP-EPM). In particular, our model allows the interaction dynamics between each pair of individuals to be modulated by their respective affiliated communities. Moreover, our model can flexibly incorporate the auxiliary individuals' attributes, or covariates associated with interaction events. Efficient Gibbs sampling and Expectation-Maximization algorithms are developed to perform inference via P\'olya-Gamma data augmentation strategy. Experimental results on real-world datasets demonstrate that our model not only achieves competitive performance for temporal link prediction compared with state-of-the-art methods, but also discovers interpretable latent structure behind the observed temporal interactions.

==> preamble_acronyms.tex <==
\newacronym{NIPS}{nips}{Neural Information Processing Systems}

==> section_experiments.tex <==



==> section_exploratory_analysis.tex <==
\section{Exploratory Analysis}
\subsection{Military interstate disputes network}
Statistical analysis of dynamic multilateral relational data, such as pairwise interactions between countries, has received a large amount of attention in recent works~\citep{hoff2016,BPTD} because these data often concern some interesting multilateral behavior of groups of countries. In this section, we investigate the interpretability of groups inferred by our model on a dynamic network of military interstate disputes (MID) between 138 countries from 1992 through 2001~\citep{MID}. Each event recored in this data set consists of four components: a sender, a receiver, the hostility level of dispute and the time coverage. We generated a dynamic network aggregating the data into monthly snapshots and created a link between each pair of two countries if either country has disputes with the other one at that given time. 
We applied our model to this dynamic network initializing the number of groups to $K=50$. Most of the identified groups correspond to some regional relations or conflicts. We select three interesting groups inferred by our model and show the group activity and the top-20 associated nodes for each of them, which confirms to our knowledge of international affairs. More specifically, we depict the group activity over time (top row) by plotting the mean of thinning function $b_k^{(t)}$. Figure~\ref{group01} shows the first group that corresponds to the second Congo war from 1998 through 2000. The six nodes with positive memberships shown in the bottom row of Figure~\ref{group01} are the belligerents of this dispute. Figure~\ref{group02} shows the second group which is mainly composed of NATO members. The activity regime of the second group confirms to the NATO bombing of Yugoslavia and the 11 associated nodes with positive memberships are indeed the belligerents of this war. Figure~\ref{group03} shows the third group which represents the regional multilateral relations among three neighbouring countries that are involved in this group with positive memberships. 

\begin{figure*} [h]
  \centering
   \begin{tabular}{ c } 
    \begin{minipage}{.75\textwidth}
      \includegraphics[width=10cm,height=8cm, keepaspectratio]{fig/comp01.pdf}
    \end{minipage}
    \\ 
      \begin{minipage}{.75\textwidth}
      \includegraphics[width=10cm,height=8cm, keepaspectratio]{fig/memberships01.pdf}
    \end{minipage}
   \end{tabular}
  \caption{The first group identified by our model on MID data corresponds to the second Congo war from 1998 through 2000 (top). We found that six countries which have positive memberships to this group are indeed the belligerents of this dispute (bottom).}
  \label{group01}
\end{figure*}

\begin{figure*} [h]
  \centering
   \begin{tabular}{ c} 
    %\vspace{5.0em}
        \begin{minipage}{.75\textwidth}
      \includegraphics[width=10cm,height=8cm, keepaspectratio]{fig/comp02.pdf}
    \end{minipage}
    \\ 
    \begin{minipage}{.75\textwidth}
      \includegraphics[width=10cm,height=8cm, keepaspectratio]{fig/memberships02.pdf}
    \end{minipage}
  \end{tabular}
  \caption{The second group inferred on MID data corresponds to the NATO bombing of Yugoslavia (top). The eleven countries associated to this group with positive memberships are indeed the belligerents of this dispute (bottom) }
  \label{group02}
%\end{table}
\end{figure*}

\begin{figure*} [h]
  \centering
   \begin{tabular}{ c } 
        \begin{minipage}{.75\textwidth}
      \includegraphics[width=10cm,height=8cm, keepaspectratio]{fig/comp03.pdf}
    \end{minipage}
    \\
    \begin{minipage}{.75\textwidth}
      \includegraphics[width=10cm,height=8cm, keepaspectratio]{fig/memberships03.pdf}
    \end{minipage}
   % \hline
  \end{tabular}
  \caption{The third group (top) inferred on MID data corresponds to the regional multilateral relations between Isreal, Lebanon and Syria (bottom).}
  \label{group03}
%\end{table}
\end{figure*}

\clearpage



\subsection{Face-to-face dynamic contacts network}

In this subsection, the inferred latent structure using our model on the face-to-face dynamic contacts (FFDC) data set described in Section 5.2 is shown for additional exploratory analysis. In figure~\ref{r_k}, the inferred group weights $r_k$ are depicted. Our model detects 9 groups totally with non-zero weights although we set $K$ to $90$ in the initialization. Figure~\ref{FFDCPlot} shows the dynamic binary adjacency matrices (column (a)), the inferred link probabilities  using our model (column (b)) and the corresponding inferred node-group association weights (column (c)). We reordered the rows and columns of the observed adjacency matrices according to the inferred node-group association weights for easier comparison. Overall, our model detects the well separated community structure that agrees with the class memberships of the students (node) presented in the FFDC data set.

\begin{figure*} [h]
  \centering
   \begin{tabular}{c } 
     %  \vspace{-2.5em}
%     \rotatebox[origin=Bc]{90}{\parbox{1.8cm}{{\scriptsize group weight $r_k$}}}
%     &
    \begin{minipage}{.75\textwidth}
      \includegraphics[width=10cm,height=5cm, keepaspectratio]{hsfig/HS180_r_k.eps}
    \end{minipage}
    \\
    %&
    {groups}
   \end{tabular}
  \caption{The inferred group weights $r_k$ using our model on face-to-face dynamic contacts data set.}
  \label{r_k}
\end{figure*}

\begin{figure*}[h]
%\begin{table}
  \centering
  \begin{tabular}{ m{0cm}  m{3.33cm}  m{3.85cm}   m{2.7cm}  m{1cm}  m{0cm}  m{0cm} m{0cm} } % { | m{-1cm}  c | c | c | c  m{-2cm} |}
   % \hline
  \vspace{-25em}
     &
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_obs_t_1.eps}
    \end{minipage}
    &
    %\begin{minipage}[t]{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_prob_t_1.eps}
    \end{minipage}
    %\end{minipage}
    & 
    %\begin{minipage}{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_membership_t_1.eps}
    \end{minipage}
    &
    %%%%
  \\
  \vspace{-25em}
  \rotatebox[origin=Bc]{90}{\parbox{3.8cm}{{\scriptsize $t_1$ }}}
    &
      \begin{minipage}{.22\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_obs_t_2.eps}
    \end{minipage}
    &
    %\begin{minipage}[t]{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_prob_t_2.eps}
    \end{minipage}
    %\end{minipage}
    & 
    %\begin{minipage}{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_membership_t_2.eps}
    \end{minipage}
    %\end{minipage}
%    &  
%    %\begin{minipage}{5cm}
%      \begin{minipage}{.25\textwidth}
%      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{synfig/DGPPF_t_6.eps}
%    \end{minipage}
%    &  
%    %\begin{minipage}{5cm}
%      \begin{minipage}{.25\textwidth}
%      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{synfig/DGPPF_t_6.eps}
%    \end{minipage}
    \\
    \vspace{-25em}
    \rotatebox[origin=Bc]{90}{\parbox{3.8cm}{{\scriptsize $t_2$ }}}
    &
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_obs_t_3.eps}
    \end{minipage}
    &
    %\begin{minipage}[t]{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_prob_t_3.eps}
    \end{minipage}
    %\end{minipage}
    & 
    %\begin{minipage}{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_membership_t_3.eps}
    \end{minipage}
    %\end{minipage}
%    &  
    %\begin{minipage}{5cm}
%      \begin{minipage}{.25\textwidth}
%      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{synfig/DGPPF_t_9.eps}
%    \end{minipage}
%    &  
%    %\begin{minipage}{5cm}
%      \begin{minipage}{.25\textwidth}
%      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{synfig/DGPPF_t_9.eps}
%    \end{minipage}
    \\
    \vspace{-25em}
    \rotatebox[origin=Bc]{90}{\parbox{3.8cm}{{\scriptsize  $t_{3}$}}}
    &
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_obs_t_4.eps}
    \end{minipage}
    &
    %\begin{minipage}[t]{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_prob_t_4.eps}
    \end{minipage}
    %\end{minipage}
    & 
    %\begin{minipage}{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_membership_t_4.eps}
    \end{minipage}
    %\end{minipage}
%    &  
%    %\begin{minipage}{5cm}
%      \begin{minipage}{.25\textwidth}
%      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{synfig/DGPPF_t_46.eps}
%    \end{minipage}
%    &  
%    %\begin{minipage}{5cm}
%      \begin{minipage}{.25\textwidth}
%      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{synfig/DGPPF_t_46.eps}
%    \end{minipage}
      \\
    \vspace{-25em}
     \rotatebox[origin=Bc]{90}{\parbox{3.8cm}{{\scriptsize $t_{4}$ }}}
    &
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_obs_t_5.eps}
    \end{minipage}
    &
    %\begin{minipage}[t]{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_prob_t_5.eps}
    \end{minipage}
    %\end{minipage}
    & 
    %\begin{minipage}{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_membership_t_5.eps}
    \end{minipage}
    %\end{minipage}
%    &  
%    %\begin{minipage}{5cm}
%      \begin{minipage}{.25\textwidth}
%      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{synfig/DGPPF_t_30.eps}
%    \end{minipage}
%    &  
%    %\begin{minipage}{5cm}
%      \begin{minipage}{.25\textwidth}
%      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{synfig/DGPPF_t_30.eps}
%    \end{minipage}
    \\
    \vspace{-25em}
     \rotatebox[origin=Bc]{90}{\parbox{3.8cm}{{\scriptsize $t_{5}$}}}
    &
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_obs_t_6.eps}
    \end{minipage}
    &
    %\begin{minipage}[t]{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_prob_t_6.eps}
    \end{minipage}
    %\end{minipage}
    & 
    %\begin{minipage}{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_membership_t_6.eps}
    \end{minipage}
    %\end{minipage}
%    &  
%    %\begin{minipage}{5cm}
%      \begin{minipage}{.25\textwidth}
%      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{synfig/DGPPF_t_43.eps}
%    \end{minipage}
%    &  
%    %\begin{minipage}{5cm}
%      \begin{minipage}{.25\textwidth}
%      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{synfig/DGPPF_t_43.eps}
%    \end{minipage}
%%%
    \\
    \vspace{-25em}
     \rotatebox[origin=Bc]{90}{\parbox{3.8cm}{{\scriptsize $t_{6}$}}}
    &
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_obs_t_7.eps}
    \end{minipage}
    &
    %\begin{minipage}[t]{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_prob_t_7.eps}
    \end{minipage}
    %\end{minipage}
    & 
    %\begin{minipage}{5cm}
      \begin{minipage}{.25\textwidth}
      \includegraphics[width=4.5cm,height=3cm, keepaspectratio]{hsfig/HS180_membership_t_7.eps}
    \end{minipage}
    \\
     \vspace{-22em}
     \rotatebox[origin=Bc]{90}{\parbox{5cm}{{\scriptsize $t_{7}$}}}
    &   \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ {\scriptsize(a)} &\  \ \ \   \ \ \  \ \ \ \ \ \ \ \ \ \ \  \ \ \ {\scriptsize(b)} &\ \ \ \ \  \ \ \  \ \ \ \ \ \ \ \ \ \ \ \ \ {\scriptsize(c)} 
%    &\ \ \ \ \ \ \ \ \ \ \ \ {\scriptsize(d)} &\ \ \ \ \ \ \ \ \ \ \ \  {\scriptsize(e)} 
    \ %\hline 
  \end{tabular}
  %\vspace{-1em}
  \caption{Dynamic community detection on face-to-face dynamic contacts data set. The adjacency matrices are shown in column (a). We reordered the rows and columns of the matrices according to the inferred node-group associations for easier visualisation. The inferred link probabilities using our model are shown in columns (b). The association weights of each node (row variable) to the latent groups (column variable) are shown in column (c). The pixel values are displayed on $\log_{10}$ scale.
}
\label{FFDCPlot}
%\end{table}
\end{figure*}



==> section_model_v2.tex <==
%\begin{align}
%\[ \def\useanchorwidth{T}\stackMath
%\lambda_{uv}(t) = \mu_{uv} + \mathop{\stackunder{\sum}{\def\stackalignment{l}%
%    {\scriptstyle j: t_j^{vu}<t}
%  }} \gamma_{kk'}(t - t_j^{vu}) \label{intensity0} \\
% = \mathop{\stackunder{\sum}{\def\stackalignment{l}%
%                    {\scriptstyle k,k'}
%  }} \mu_{ukk'v} + \mathop{\stackunder{\sum}{\def\stackalignment{l}%
%    \stackunder[2pt]{\scriptstyle j: t_j^{vu}<t}
%                    {\scriptstyle z_v = k', z_u = k}
%  }} \alpha_{kk'}\exp(-\delta(t - t_{j}^{vu}))\]
%  
%  \[ %\def\useanchorwidth{T}\stackMath
%\lambda_{uv}(t) = \mu_{uv} + {\stackunder{\sum}{\def\stackalignment{l}%
%    {\scriptstyle j: t_j^{vu}<t}
%  }} \gamma_{kk'}(t - t_j^{vu}) \label{intensity0} \\
% = \mathop{\stackunder{\sum}{\def\stackalignment{l}%
%                    {\scriptstyle k,k'}
%  }} \mu_{ukk'v} + \mathop{\stackunder{\sum}{\def\stackalignment{l}%
%    \stackunder[2pt]{\scriptstyle j: t_j^{vu}<t}
%                    {\scriptstyle z_v = k', z_u = k}
%  }} \alpha_{kk'}\exp(-\delta(t - t_{j}^{vu}))\]
%\end{align}
%\begin{align}

%\[\def\useanchorwidth{F}\stackMath
%\begin{aligned}
%\lambda_{uv}(t) & = \mu_{uv} + {\stackunder{\sum}{\def\stackalignment{l}%
%    {\scriptstyle j : t_j^{vu}<t}
%  }} \gamma(t - t_j^{vu}) \label{intensity}\\
%& = {\stackunder{\sum}{\def\stackalignment{l}%
%                    {\scriptstyle k,k'}
%  }} \mu_{ukk'v} + {\stackunder{\sum}{\def\stackalignment{l}%
%                    {\scriptstyle k,k'}
%  }} \mathop{\stackunder{\sum}{\def\stackalignment{l}%
%    \stackunder[2pt]{\scriptstyle j: t_j^{vu}<t}
%                    {\scriptstyle z_v = k', z_u = k}
%  }} \alpha_{kk'}\exp(-\delta(t - t_{j}^{vu})), \notag
%\end{aligned}
%\]



==> section_relatedworks.tex <==
\

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=22pt, font=\fontsize{12}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=2pt, fit=#1]

\tikzstyle{newwrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
above right=0pt and 0pt of #1.north east] %
\tikzstyle{new plate caption} = [caption, node distance=0, inner sep=0pt,
above right=0pt and 0pt of #1.south west] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[-,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[newwrap=#3] (#2-newwrap) {}; %
  \node[plate caption=#2-newwrap] (#2-caption) {#4}; %
  \node[plate=(#2-newwrap)(#2-caption), #1] (#2) {}; %
}

\newcommand{\newplate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[new plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


